HMP: Hand Motion Priors for Pose and Shape Estimation from Video

Understanding how humans interact with the world necessitates accurate 3D hand pose estimation, a task complicated by the hand's high degree of articulation, frequent occlusions, self-occlusions, and rapid motions. While most existing methods rely on single-image inputs, videos have useful cues to address aforementioned issues. However, existing video-based 3D hand datasets are insufficient for training feedforward models to generalize to in-the-wild scenarios. On the other hand, we have access to large human motion capture datasets which also include hand motions, e.g. AMASS. Therefore, we develop a generative motion prior specific for hands, trained on the AMASS dataset which features diverse and high-quality hand motions. This motion prior is then employed for video-based 3D hand motion estimation following a latent optimization approach. Our integration of a robust motion prior significantly enhances performance, especially in occluded scenarios. It produces stable, temporally consistent results that surpass conventional single-frame methods. We demonstrate our method's efficacy via qualitative and quantitative evaluations on the HO3D and DexYCB datasets, with special emphasis on an occlusion-focused subset of HO3D. Code is available at https://hmp.is.tue.mpg.de

==> figures/keypoint_fail.tex <==
\twocolumn[{%
	\renewcommand\twocolumn[1][]{#1}%
	\maketitle
	\begin{center}
		\newcommand{\teaserwidth}{\linewidth}
		% \vspace{-0.15in}
		\centerline{
			\includegraphics[width=\teaserwidth,clip]{figures/pdf_files/keyp_failure_wo_rgb.pdf}
		}
		% \vspace{-1ex}
		\captionof{figure}{\textbf{Estimation of \methodname under faulty keypoint detections. Left: 2d keypoints from \cite{pymafx2022}, middle and right \cite{lugaresi2019mediapipe}}

		% \vspace{-0.08in}
		\label{fig:in_the_wild_qual}
	\end{center}%
}]

==> main.tex <==
% \input{main_review}
\input{main_camera_ready}
% \input{main_supmat}



==> tables/motion_prior_ablation.tex <==
\begin{table*}[tb]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|r|r|r|r|r|r|r|r}
        \toprule
        & \multicolumn{2}{c|}{\textbf{HO3D-v3}} & \multicolumn{2}{c|}{\textbf{DexYCB}} & \multicolumn{2}{c|}{\textbf{Runtime}}
        \\
        \textbf{Methods} & \textbf{\procrustesAlignedErr} $\downarrow$ & \textbf{\rootAlignedErr} $\downarrow$ & \textbf{\procrustesAlignedErr} $\downarrow$ & \textbf{\rootAlignedErr} $\downarrow$ & \textbf{128 frames} $\downarrow$ & \textbf{1024 frames} $\downarrow$ 
        \\ 
        \midrule 
        No Motion Prior & 10.5 & 28.0 & 10.9 & 36.4 & 33s & 46s 
        \\ 
        PCA-based & 13.8 & 31.1 & 16.9 & 41.6 & 40s & 58s
        \\
        GMM-based & 10.4 & 27.5 & 10.8 & 38.6 & 1m 24s & 9m 9s
        \\ 
        \acronym HMP (Ours) & \textbf{10.0} & \textbf{26.8} & \textbf{8.9} & \textbf{34.1} & 35s & 54s
        \\ 
        \bottomrule
        \end{tabular}
        }
   % \vspace{-2mm}
   \caption{Ablation study with different motion priors on HO3D-v3 and Dex-YCB datasets \cite{hampali2021ho3dv3, chao2021dexycb}.}
   % \vspace{-4mm}
   \label{tab:mp_ablation}
\end{table*}


==> tables/motion_prior_runtime_diversity.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|r|r|r|r|r|r|r|r}
        \toprule
        & \multicolumn{2}{c|}{\textbf{HO3D-v3}} & \multicolumn{2}{c|}{\textbf{DexYCB}} & \multicolumn{2}{c|}{\textbf{Runtime $\downarrow$}}
        \\
        \textbf{Methods} & \textbf{\procrustesAlignedErr} $\downarrow$ & \textbf{\rootAlignedErr} $\downarrow$ & \textbf{\procrustesAlignedErr} $\downarrow$ & \textbf{\rootAlignedErr} $\downarrow$ & 128 frames & 1024 frames   
        \\ 
        \midrule 
        No Motion Prior & 10.5 & 28.0 & 10.9 & 36.4 & 33s & 46s
        \\ 
        PCA-based & 13.8 & 31.0 & 16.9 & 41.6 & 40s & 58s
        \\
        GMM-based & 10.3 & 27.3 & 10.8 & 38.6 & 1m 24s & 9m 9s 
        \\ 
        \acronym HMP (Ours) & \textbf{10.0} & \textbf{26.8} & \textbf{8.9} & \textbf{34.1} & 35s & 54s
        \\ 
        \bottomrule
        \end{tabular}
        }
   \vspace{-2mm}
   \caption{Ablation study with different motion priors on HO3D-v3 and Dex-YCB datasets \cite{hampali2021ho3dv3, dexycb}.}
   \vspace{-4mm}
   \label{tab:mp_ablation}
\end{table*}

